Achievable Fairness on Your Data With Utility Guarantees

In machine learning fairness, training models that minimize disparity across different sensitive groups often leads to diminished accuracy, a phenomenon known as the fairness-accuracy trade-off. The severity of this trade-off inherently depends on dataset characteristics such as dataset imbalances or biases and therefore, using a uniform fairness requirement across diverse datasets remains questionable. To address this, we present a computationally efficient approach to approximate the fairness-accuracy trade-off curve tailored to individual datasets, backed by rigorous statistical guarantees. By utilizing the You-Only-Train-Once (YOTO) framework, our approach mitigates the computational burden of having to train multiple models when approximating the trade-off curve. Crucially, we introduce a novel methodology for quantifying uncertainty in our estimates, thereby providing practitioners with a robust framework for auditing model fairness while avoiding false conclusions due to estimation errors. Our experiments spanning tabular (e.g., Adult), image (CelebA), and language (Jigsaw) datasets underscore that our approach not only reliably quantifies the optimum achievable trade-offs across various data modalities but also helps detect suboptimality in SOTA fairness methods.

==> macros.tex <==
%
\RequirePackage{snapshot}
\usepackage{subcaption}
%
\usepackage{caption}
\usepackage{graphicx}
\usepackage{comment}
%
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{thmtools,thm-restate}
\usepackage{bbm}
\usepackage{mathtools}
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
%
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\usepackage{tikz}
\usepackage{wrapfig}
\usepackage{titletoc}
\usepackage[page,header]{appendix}


\newcommand{\calH}{\mathcal{H}}
\newcommand{\FairViolation}{\textbf{M}\,\boldsymbol{\mu}}
\newcommand{\Err}{\textup{err}}
%
%
\newcommand{\BestH}{\textup{BEST}_{h}}
\newcommand{\Bestlambda}{\textup{BEST}_{\lambda, \textbf{v}}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\linf}[1]{||#1||_\infty}
\newcommand{\ind}{\mathbbm{1}}
\newcommand{\fairnessloss}{\Phi_{\textup{fair}}}
\newcommand{\tradeoff}{\tau^\ast_{\textup{fair}}}
\newcommand{\fairnesslossrelaxed}{\mathcal{L}_{\textup{fair}}}
\newcommand{\celoss}{l_{\textup{CE}}}
\newcommand{\errinterval}{R^\alpha_{\textup{err}}}
\newcommand{\accinterval}{R^\alpha_{\textup{acc}}}
\newcommand{\fairnessinterval}{R^\alpha_{\textup{fair}}}
\newcommand{\fairnessintervalup}{U^{h}_{\textup{fair}}}
\newcommand{\fairnessintervallo}{L^{h}_{\textup{fair}}}
\newcommand{\accintervalup}{U^{ h}_{\textup{acc}}}
\newcommand{\accintervallo}{L^{ h}_{\textup{acc}}}
\newcommand{\fairnessintervaluplambda}{U^{\lambda}_{\textup{fair}}}
\newcommand{\fairnessintervallolambda}{L^{\lambda}_{\textup{fair}}}
\newcommand{\accintervaluplambda}{U^{\lambda}_{\textup{acc}}}
\newcommand{\accintervallolambda}{L^{\lambda}_{\textup{acc}}}
%
%
\newcommand{\fairnesslowtilde}{\tilde{L}^\alpha_{\textup{f}}}
\newcommand{\fairnessuptilde}{\tilde{U}^\alpha_{\textup{f}}}
\newcommand{\Xt}{\tilde{X}}
\newcommand{\At}{\tilde{A}}
\newcommand{\Yt}{\tilde{Y}}
\newcommand{\Ah}{\hat{A}}
\newcommand{\Dt}{\tilde{\mathcal{D}}}
\newcommand{\True}{\textup{True}}
\newcommand{\simiid}{\overset{\text{iid}}{\sim}}
%
%
%
\newcommand{\Acc}{\textup{acc}}
%
\newcommand{\fairnessintervalset}{C_{\textup{fair}}}
\newcommand{\accintervalset}{C_{\textup{acc}}}
\newcommand{\tr}{\textup{tr}}
\newcommand{\Dtr}{\mathcal{D}^{\tr}}
\newcommand{\Xtr}{X^{\tr}}
\newcommand{\Atr}{A^{\tr}}
\newcommand{\Ytr}{Y^{\tr}}
\newcommand{\Yh}{\hat{Y}}
%
%
\newcommand{\dpmetric}{\Phi_\textup{DP}}
\newcommand{\eopmetric}{\Phi_\textup{EOP}}
\newcommand{\eometric}{\Phi_\textup{EO}}
\newcommand{\caldata}{\mathcal{D}_{\textup{cal}}}
\newcommand{\trdata}{\mathcal{D}_{\textup{tr}}}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\tradeoffCIs}{\Gamma_{\textup{fair}}}
\newcommand{\surrogatemodel}{f_{\mathcal{A}}}

\newcommand{\squishlist}{
\begin{list}{{{\small{$\bullet$}}}}
{\setlength{\itemsep}{1pt}      \setlength{\parsep}{0pt}
\setlength{\topsep}{-2pt}       \setlength{\partopsep}{0pt}
\setlength{\leftmargin}{1em} \setlength{\labelwidth}{1em}
\setlength{\labelsep}{0.5em} } }
\newcommand{\squishend}{  \end{list}  }
\DeclareMathOperator*{\argmin}{arg\,min}

\renewcommand{\eqref}[1]{Eq.~(\ref{#1})}
\newcommand{\trsize}{|\trdata|}
%

%

%
\usepackage{colortbl}


%
%
%
%

\usepackage[compact]{titlesec}
%
%
\titlespacing{\subsubsection}{0pt}{*0}{*0}
\titlespacing{\paragraph}{0pt}{*0}{*0.8}
\usepackage{multirow}

\urlstyle{same}
